Distributed Technology-Sustained Pervasive Applications

Technology-sustained pervasive games, contrary to technology-supported pervasive games, can be understood as computer games interfacing with the physical world. Pervasive games are known to make use of 'non-standard input devices' and with the rise of the Internet of Things (IoT), pervasive applications can be expected to move beyond games. This dissertation is requirements- and development-focused Design Science research for distributed technology-sustained pervasive applications, incorporating knowledge from the domains of Distributed Computing, Mixed Reality, Context-Aware Computing, Geographical Information Systems and IoT. Computer video games have existed for decades, with a reusable game engine to drive them. If pervasive games can be understood as computer games interfacing with the physical world, can computer game engines be used to stage pervasive games? Considering the use of non-standard input devices in pervasive games and the rise of IoT, how will this affect the architectures supporting the broader set of pervasive applications? The use of a game engine can be found in some existing pervasive game projects, but general research into how the domain of pervasive games overlaps with that of video games is lacking. When an engine is used, a discussion of, what type of engine is most suitable and what properties are being fulfilled by the engine, is often not part of the discourse. This dissertation uses multiple iterations of the method framework for Design Science for the design and development of three software system architectures. In the face of IoT, the problem of extending pervasive games into a fourth software architecture, accommodating a broader set of pervasive applications, is explicated. The requirements, for technology-sustained pervasive games, are verified through the design, development and demonstration of the three software system architectures. The ...

==> includes/0_ignorance.tex <==
%!TEX root = ../manuscript.tex

% this file is called up by thesis.tex
% content in this file will be fed into the main document

%: ----------------------- introduction file header -----------------------

\graphicspath{{includes/0_img/}} % specifies where the figures are stored

% ----------------------------------------------------------------------
%: ----------------------- content ----------------------- 
% ----------------------------------------------------------------------

\section*{The Five Orders of Ignorance~\normalsize{\cite[original bold]{armour2000-5oi}}}

\noindent``Since we are computer folk, we start counting from zero, rather than one. \dots
\begin{description}
\item[0th Order Ignorance (0OI)-- Lack of Ignorance.] \hfill \break
I have 0OI when I know something and can demonstrate my lack of ignorance in some tangible form, \dots

\item[1st Order Ignorance (1OI)-- Lack of Knowledge.] \hfill \break
I have 1OI when I don't know something and can readily identify that fact. 1OI is basic ignorance. \dots

\item[2nd Order Ignorance (2OI)-- Lack of Awareness.] \hfill \break
I have 2OI when I don't know that I don't know something. 
That is to say, not only am I ignorant of something (for instance I have 1OI), I am unaware of this fact. I don't know enough to know that I don't know enough. \dots

\item[3rd Order Ignorance (3OI)-- Lack of Process.] \hfill \break
I have 3OI when I don't know a suitably efficient way to find out I don't know that I don't know something. \dots\xspace
If I have 3OI, I don't know of a way to find out there are things I don't know that I don't know. Therefore, I can't change those things I don't know that I don't know into either things that I know, or at least things I know that I don't know, as a step toward converting the things I know that I don't know into things I~know. \dots

\item[4th Order Ignorance (4OI)-- Meta Ignorance.] \hfill \break
I have 4OI when I don't know about the Five Orders of Ignorance. 
I~no~longer have this kind of ignorance, and now, neither, dear reader, do~you.''

\end{description}

% ---------------------------------------------------------------------------
%: ----------------------- end of thesis sub-document ------------------------
% ---------------------------------------------------------------------------


